D-STACK: High Throughput DNN Inference by Effective Multiplexing and Spatio-Temporal Scheduling of GPUs

Hardware accelerators such as GPUs are required for real-time, low-latency inference with Deep Neural Networks (DNN). However, due to the inherent limits to the parallelism they can exploit, DNNs often under-utilize the capacity of today's high-end accelerators. Although spatial multiplexing of the GPU, leads to higher GPU utilization and higher inference throughput, there remain a number of challenges. Finding the GPU percentage for right-sizing the GPU for each DNN through profiling, determining an optimal batching of requests to balance throughput improvement while meeting application-specific deadlines and service level objectives (SLOs), and maximizing throughput by appropriately scheduling DNNs are still significant challenges. This paper introduces a dynamic and fair spatio-temporal scheduler (D-STACK) that enables multiple DNNs to run in the GPU concurrently. To help allocate the appropriate GPU percentage (we call it the "Knee"), we develop and validate a model that estimates the parallelism each DNN can utilize. We also develop a lightweight optimization formulation to find an efficient batch size for each DNN operating with D-STACK. We bring together our optimizations and our spatio-temporal scheduler to provide a holistic inference framework. We demonstrate its ability to provide high throughput while meeting application SLOs. We compare D-STACK with an ideal scheduler that can allocate the right GPU percentage for every DNN kernel. D-STACK gets higher than 90 percent throughput and GPU utilization compared to the ideal scheduler. We also compare D-STACK with other GPU multiplexing and scheduling methods (e.g., NVIDIA Triton, Clipper, Nexus), using popular DNN models. Our controlled experiments with multiplexing several popular DNN models achieve up to 1.6X improvement in GPU utilization and up to 4X improvement in inference throughput.

==> sections/Primitives.tex <==
\vspace{-1mm}\section{Primitives in GPU Runtime Software for Enhanced Performance}\vspace{-1mm}
%\vspace{-1mm}
GPU runtimes are optimized for launching long-running applications reading bulk-data from disk. Often time, they are inefficient while running real-time applications working with streaming data. We describe primitives, which makes running real-time inference using DNN models more efficient. 
\subsection{Improving CPU-GPU Co-ordination}\vspace{-2mm} %\knote{this comes at the wrong place. It is better to put it after the next subsection on modeling the DNN parallelism. This way, we can segue to the OS primitives section.}

%Moreover, 
\begin{figure*}
\vspace{-2mm}
    \centering
    \subfloat[Mobilenet with 100\% GPU (1 ms profile)]{
    \includegraphics[width=.40\linewidth]{figures/DNN_Profiles/mobilenet_100p_1ms.png}
    %\caption{}
    \label{fig:mobilenet_1ms_100p}}
    \subfloat[Mobilenet (15\% GPU)]{
    \includegraphics[width=.24\linewidth]{figures/DNN_Profiles/mobilenet_15p_1ms_small.png}
    %\caption{PyTorch Mobilenet (15\% GPU) 1 ms inference profile}
    \label{fig:mobilenet_1ms_15p}}
    \subfloat[ResNet-18: CPU wait time\Scut{between 2 inferences}]{
    \includegraphics[width=.31\linewidth]{figures/DNN_Profiles/Resnet-18_two_profiles.png}
    \label{fig:resnet18_1_image_inference}
    }
    \vspace{-4mm}
    \caption{Inference profiles (snapshot from NVPROF tool, 1 millisecond for (a) and (b), 3 ms for (c)) for different DNN models on PyTorch.}
    \vspace{-4mm}
\end{figure*}

%\begin{figure*}
%    \centering
    %\subfloat[GNMT Thread Count for 25 Word inference. There are 74 kernels so I am coloring few of most recurring ones.]{
%    \includegraphics[width=\linewidth]{figures/GNMT_data/twenty_five_words/latency_threads_gnmt.pdf}
%    \caption{GNMT Thread Count for 25 Word inference}
%    \label{fig:GNMT_thread_count}
    
%\end{figure*}

\update{
GPU operations are executed asynchronously with respect to the CPU. GPUs maintain a queue where the GPU's runtime API calls and kernel launches are en-queued for subsequent GPU processing. This queuing helps to free up the CPU after submitting the job to GPU and allows a single CPU thread to submit multiple tasks to GPU without waiting for the completed tasks. DNN models are composed of multiple GPU kernels sequentially processing an input. ML platforms such as TensorFlow, PyTorch \etc \Scut{offer user-friendly API and abstract the multiple kernel launches, but, internally, the ML platforms }launch all the model's kernels asynchronously. However, \Scut{we have observed that} asynchronous launches adversely impact the inference latency and utilization of GPU resources. 

\Scut{We have observed that even a lightweight DNN model such as Mobilenet requires a few hundred DNN kernel executions for a single inference operation.} Fig.~\ref{fig:mobilenet_1ms_100p} shows the CPU-GPU profile for DNN inference using the Mobilenet model in PyTorch with 100\% GPU. 
We only extracted a one millisecond time slice out of the whole profile to depict CPU and GPU's finer granularity behavior. This profile shows the idle time between executions of CUDA runtime functions in CPU, \emph{and} the idle time in the GPU compute timeline. These idle times are caused by the inefficient launching of DNN kernels by the ML platform. We also present the Mobilenet inference profile with 15\% GPU in Fig.~\ref{fig:mobilenet_1ms_15p}. We can still observe the gaps in CPU and GPU to exist, but DNN kernels are now running slower with only 15\% GPU available. These slower kernels utilize the gaps between the two kernel execution and do not increase the overall task completion time, even at this low GPU\%. We should note that DNN with compute-heavy kernels that run longer do not show as much of a gap between consecutive GPU kernel executions. Longer DNN kernel executions in the GPU means that the CPU thread calling the runtime API finishes launching the kernels asynchronously before the GPU completes running all the DNN kernels. Therefore, the effect of CPU-GPU co-ordination is more pronounced in DNN models with kernels that have short runtime.

Ideally, all the GPU kernels in the ML platform should be launched asynchronously. There are a number of different components that contribute to latency of DNN inference. Having an adequate proportion of the GPU allocated is important to keep the latency low. However, a number of other design decisions contribute significantly to the latency. One is the time taken to launch the DNN kernel. This requires careful CPU-GPU coordination to launch the DNN kernels together with the runtime of the constituent kernels as discussed in \S~\ref{limits_on_parallelism} to reduce this latency. We address in this subsection.

\Scut{
However, since the CPU/GPU runtime has significant latency in launching DNN kernels, running DNN models at a lower GPU\% does not significantly increase the overall latency \knote{this doesn't follow - latency to launch doesn't imply running at lower GPU doesn't have impact. Rewrite}. %These observations demonstrate that 
The latency of inference is also dependent on CPU-GPU co-ordination .  These findings further encourage using controlled spatial sharing to limit the DNN to certain GPU resources and still obtain good DNN processing latency. 
\knote{this paragraph doesn't make a lot of sense Aditya. You just want to say -  4 sentences should be enough.}
}
}

\Scut{
GPU operations can be executed asynchronously with respect to the CPU. GPUs maintain a queue where runtime API calls and kernel launches from applications running in the CPU can be en-queued for subsequent GPU processing. This helps to free up the CPU after submitting the job to GPU and also allows a single CPU thread to submit multiple tasks to GPU without waiting for the tasks to be completed. ML platforms such as TensorFlow, PyTorch \etc %abstract out the low level CUDA / CuDNN API and 
offer user-friendly APIs %\Scut{\sknote{What are these APIs? CuDDNs?}} to construct a DNN model by specifying the layers, %constructed out of "layers". 
and abstract out the low-level (GPU kernel level CUDA/CuDNN) execution details.
%\sknote{Please check if the above sentence is a correct interpretation? Correct. Will remove the comment}
Asynchronous kernel launches allow CPU threads to launch all DNN kernels quickly without waiting for feedback from GPU.
\Scut{However, when the DNN is run on the GPU, it is often executed sequentially, by executing each of the large number of GPU kernels one layer after another, with the CPU involved in the initiation of each DNN (CUDA) kernel. This requirement of multiple kernel launches for running a single DNN as well as } 
However, this brings up CPU-GPU co-ordination challenges that can adversely impact the inference latency and utilization of GPU resources.
%asynchronous nature of CPU-GPU co-ordination brings up challenges while performing inference using DNN as CPU does not have information on beginning and ending of certain tasks.

%There are many tasks that execute serially on the GPU %\knote{you mean that phases are serialized? rather than non-parallelizable tasks?} 
%during the DNN inference process. 

%by layer fashion. And, %as multiple CUDA kernels and 
%For each DNN layer's operation, the CPU initiates the execution of a CUDA kernel one after another, in a sequential manner.  %might be performed by set os in f CUDA kernels. 
%\anote{I think this can be removed.}
%\knote{agreed}
\Scut{
Each of these DNN kernels are launched by a CPU program, and each kernel launch-process also adds to the latency. 
Each of the DNN kernels also have to load instructions into the SMs, read weights for the DNN and write the output of their computation to a specific GPU memory location, which also adds to the latency. 
These kernel operations are serialized with rest of DNN processing.
}
%\anote{till here}

Even lightweight DNNs such as Mobilenet require a few hundred DNN kernel executions for a single inference operation. Fig.~\ref{fig:mobilenet_1ms_100p} shows the CPU-GPU profile for DNN inference using the Mobilenet model in PyTorch with 100\% GPU. 
We only extracted a one millisecond time slice out of the whole profile to clearly depict the finer granularity behavior of CPU and GPU usage. 
This profile shows the idle time between executions of CUDA runtime functions in CPU, \emph{and} the idle time in the GPU compute timeline as well. These idle times are caused by the inefficient launching of DNN kernels by ML platform. 
ML platforms such as PyTorch call numerous additional CUDA API functions to check for GPU execution errors and also for checking the GPU device error and status before launching the subsequent DNN kernel. For DNNs with kernels that run for a very short time, this delay in the CPU launch of the kernel causes the GPU to be idle for a large fraction of overall DNN inference time. Note the GPU is idle when the CPU is busy. 
We also present the Mobilenet inference profile with 15\% GPU in Fig.~\ref{fig:mobilenet_1ms_15p}. We can still observe the gaps in CPU and GPU  to exist, but, DNN kernels now are being run slower with only 15\% GPU available. These slower kernels utilize the gaps between the two kernel execution and also do not increase the overall task completion time even at this low GPU\%. 
Ideally, it would be good to have ML platform launch all the GPU kernels asynchronously at once. However, in cases where CPU might be slow at launching DNN kernels, the lower GPU\% does not impact the inference latency significantly. Further, this mode allows us to share and utilize the remaining GPU across the other applications concurrently.%\looseness-1
%The remaining GPU may be used for other applications to use it concurrently. %as 100\% GPU by utilizing the idle time created by slow DNN kernel launches.  

We also observe that DNN with compute-heavy kernels that run longer do not show as much of a gap between consecutive GPU kernel executions. Longer DNN kernel executions in the GPU means that the CPU thread calling the runtime API finishes launching the kernels asynchronously before the GPU completes running all the DNN kernels.
\Scut{Moreover, in DNN with kernels that run in the GPU for longer, the CPU execution of CUDA runtime functions ends much earlier than the DNN processing as seen in a} Fig.~\ref{fig:resnet18_1_image_inference} shows the profile of inference with ResNet-18, that shows large amount of CPU time being spent on running (actually being blocked on) an API function \textit{cudaDeviceSynchronize()}.   %before finishing DNN computation in GPU.. This creates a situation 
During the execution of this function, the CPU waits for the GPU to complete processing the kernel and return the result. By avoiding this waiting, we can utilize the idle CPU for other tasks. To achieve this wait-free CPU execution and to achieve low latency inference, it is highly desirable to have a timely notification of task completion. 

}
%\sknote{The figure does not seem to show the idle time to be an issue nor make a point for timely notification. Infact the idle time shown in the figure seems desirable. I think, it will be better to show the CPU idel time as a gap between when the GPU ends, and when the CPU actually becomes busy next. Please check!! }\anote{See now. Unfortunately, the profiler sees the gap as API call getting executed.}


\Scut{Thus, the latency to complete these operations cannot be lowered by just providing more GPU resources.
\sknote{is it possible to get the CPU time expended for performing this operation and compare to the actual GPU execution time for the MobileNet to show the overhead factor?}}

%\begin{itemize}
%    \item 
\Scut{
\begin{enumerate}
    \item The CPU and GPU processing streams can be asynchronous and should be able to run in parallel. To provide a notification of GPU task completion, we can put callback after each inference is completed. However, we find that such callbacks are not effective in multiplexing scenarios.
This is because a callback blocks all the subsequent CPU work on the stream that launched the callback as well as other concurrently running streams until the callback is processed. Therefore, it introduces delays on the other execution stream.
    \item The callback blocks the execution of CUDA API. Therefore, if it is used to notify the end of inference, we still need to switch the context to another thread before executing in GPU again.
    \item Lightweight monitoring is available by putting a "CUDA Event:" as a flag towards the end. \knote{so what?} 
\end{enumerate}
}
\textbf{Task Completion Notification}:
%\knote{get rid of the itemization}
%\Scut{As we noted earlier, there are a number of serialized operations with the GPU tasks invoked by a function running on the CPU. It is very desirable that both the CPU and GPU operations proceed in parallel, to get better resource utilization, reduce CPU and GPU idle time and get better overlap between CPU and GPU specific tasks. Overall this has the effect of improving throughput and possibly reducing inference latency.}
%GPU operations can be executed asynchronously with respect to the CPU. This helps to free up the CPU after submitting the job to GPU and also allows a single CPU thread to submit multiple tasks to GPU without waiting for the tasks to be completed. 
%in multiple streams which will be performed asynchronously without blocking the CPU.
\update{Due to asynchronous nature of GPU kernels, there is no simple way for the CPU to know when tasks submitted to GPU has completed. One of the method to reduce overhead of notification of completion and launch of subsequent task in GPU is to use \textit{Graph APIs} such as CUDA Graph available in major GPU runtimes. Graph APIs allows programmer to define an execution graph for GPU kernels with their dependencies. However, CUDA graph is designed for running same workload repeatedly and is not flexible to accommodate applications that have dynamic scheduling, requiring rebuilding of graph on the fly. Furthermore, CUDA Graph needs the kernels in graph be launched from same CPU process. Therefore, in our system, where DNN models are run in different applications/ML platforms, use of CUDA graph to organize execution workflow is not possible. 

Other method for notification of work completion in GPU is to put explicit synchronization barriers between CPU and GPU and to wait for GPU to finish the given work. Fig.~\ref{fig:resnet18_1_image_inference} shows the profile of inference with ResNet-18, that shows large amount of CPU time being spent on running (actually being blocked on) an API function \textit{cudaDeviceSynchronize()}. Explicit synchronization idles the CPU for a long time while waiting for the kernel to complete and return the result. Yet another method is to use a \textit{callBack} API to notify end of execution of a kernel by invoking a callback. However, the current implementation of the callbacks poses challenges for GPU multiplexing. First, \Scut{until the completion of the execution of the} callback routine blocks all the subsequent execution on the GPU until the callback is resolved, resulting in the idling of the GPU. Second, the callback context on the CPU is forbidden from invoking any of the CUDA APIs. Thus, callback can only function as signal that some task ended in GPU but cannot launch the pending GPU related tasks. This limitation requires an additional CPU context and signaling scheme to perform any GPU related operations. 

To overcome these limitations, we devise a lightweight method for the CPU to obtain the GPU task completion status. 
We leverage CUDA's event APIs to record an 'event' (this can be per GPU stream) when the DNN execution completes. \Scut{The CUDA event acts as a flag. When executed by the GPU, it records the time of the execution.} The CUDA API function \textit{cudaEventRecord()} allows us to put an event marker at the end of the DNN's execution. We can then use another API function \textit{cudaEventQuery()} to check if the event that we placed has been executed or not. Using this event method also helps us avoid the CPU thread blocking caused by callbacks and allows to start different GPU tasks within the same CPU thread context. Our event checking is lightweight, taking about 2 $\mu$seconds in our system. 
As the DNNs usually take a few milliseconds to perform an inference, we check the event at a relatively interval of 100 micro-second to find out when the DNN computation has ended, thus, providing the flexibility for the CPU thread to check event completion status at a desired frequency.

To evaluate the improvement, we ran inference (Alexnet on TensorRT) with callback and our notification approaches. The Callback approach added $\sim$600$\mu$s idle time on GPU, resulting in a 4.1 ms  average inference latency. The event based approach had an avg. inference latency of 3.4 ms \ie \textbf{(17\% faster)}. 
%While 600$\mu$s is not a significant fraction of time for inferring with heavier model, it is a significant amount of time for latency of lighter models. 
Effective task completion notification allows a relatively larger benefit for inference, especially with lighter models.  
}
\Scut{ 
ML platforms put explicit synchronization barriers between CPU and GPU by using synchronization API to wait for GPU to finish the given work. 
ML platforms also use implicit synchronization APIs in CUDA (\eg PyTorch uses \textit{cudaMalloc} %\sknote{by PyTorch? or MXNet? whom?}\anote{Pytorch, I am not yet sure about MxNet}
) that makes CPU wait till the corresponding CUDA API call is executed. 
Synchronization barriers cause CPU to idle while waiting for the synchronization event.
Alternatively, ML Platforms can also leverage the asynchronous CUDA APIs to avoid blocking of the CPU task on the synchronization events.
Although asynchronous execution helps free the CPU thread from getting blocked, %and wait for completion of the GPU task, %due to asynchronous execution, 
there is no simple way for the CPU task to know when a submitted task has completed on the GPU. 

The CUDA API offers \textit{cudaStreamAddCallback()},  a 'callback' function to notify the end of processing in the GPU by running a callback function on the CPU. %It can run a CPU side function after a number of submitted tasks on the GPU have completed. %This callback can be used to notify the end of processing in the GPU. 
%Although the callback helps notify the end of a particular task, 
However, the current implementation of the callback poses challenges for GPU multiplexing. 
First, until the completion of the execution of the callback routine on the CPU, it blocks all the subsequent execution on the GPU resulting in the idling of the GPU. % and the CPU thread that the callback uses. 
\Scut{The callback execution can also block other streams which also use the same CPU thread blocked by the callback, to feed tasks to the GPU or to execute their own callbacks. Repeated callbacks from different streams results in the GPU idling.} 
%Second, callback functions generated by the GPU forbid the CPU thread to run any of the CUDA API functions. 
Second,  the callback context on the CPU is forbidden from invoking any of the CUDA APIs.
This limitation requires an additional CPU context and signaling scheme to perform any GPU related operations. 
That is, the callback can signal the end of computation in the GPU, but the same callback function cannot be used to transfer the result back to host memory or start another computation in GPU since that requires launching a CUDA API. 
%To run something else in the GPU, the callback has to end and a CPU thread has to run without the callback context.
Hence, the callback approach with CUDA results in lower GPU utilization due to idling, It also incurs complexity in case the CPU needs to perform any GPU related operations in the callback context.%\looseness-1 %the reduce the GPU utilization by idling it, as well as limit the CPU in performing GPU related actions.  
%\knote{I am wondering if this para is too long. But I don't know how to cut it short. Sameer?}\sknote{I have updated, cut a bit and may be elongated a bit too.} 

To overcome these limitations, we devise a lightweight method for the CPU to obtain the GPU task completion status. 
We leverage CUDA's event APIs to record an 'event' (this can be per GPU stream) when %\knote{is it 'when' not 'where'?}
the DNN execution completes. The CUDA event acts as a flag. When executed by the GPU, it records the time of the execution. The CUDA API function \textit{cudaEventRecord()} allows us to put an event marker at the end of the DNN's execution. We can then use another API function \textit{cudaEventQuery()} to check if the event that we placed has been executed or not. 
This allows us to not only avoid the idling of the GPU, but also provide the flexibility to perform different GPU tasks within the same CPU thread context. 
%Moreover, 
Our event checking is lightweight, taking about 2 $\mu$seconds in our system. 
As the DNNs usually take a few milliseconds to perform an inference, we check the event at a relatively interval of 100 micro-second to find out when the DNN computation has ended, thus %Hence, this approach also 
providing the flexibility for the CPU thread to check event completion status at a desired frequency. %\looseness-1 
%An execution of the event means the kernels that were placed in stream before the event, \ie DNN kernels, have completed  execution. This lets us know the completion of the DNN. The event checking is very lightweight and only requires about 5 $\mu$seconds in our testbed. As the DNNs we use usually take milliseconds to perform an inference, we check the event with a coarse interval of 1 milli-seconds to find out when the DNN computation has ended. 
Using this event method helps us avoid the CPU thread blocking caused by callbacks. It also avoids the callback context, and therefore lets us instantly launch another task in GPU after a particular task has completed.

To evaluate the improvement, we ran inference (Alexnet on TensorRT) with callback and our notification approaches. 
The Callback approach added $\sim$600$\mu$s idle time on GPU, resulting in a 4.1 ms  average inference latency. The event based approach had an  avg. inference latency of 3.4 ms \ie \textbf{(17\% faster)}. 
%While 600$\mu$s is not a significant fraction of time for inferring with heavier model, it is a significant amount of time for latency of lighter models. 
Eliminating callback provides a relatively larger benefit for inference, especially with lighter models.  
}
%\knote{Show evidence of benefit}    
\Scut{
    Uncontrolled spatial sharing of the GPU results in unpredictable latency for applications executing in the GPU \knote{doesn't have anything to do with task completion}. Knowing when the task ends is crucial for deadline based systems \knote{not relevant}. To ensure that we know when a DNN inference that runs in GPU can end we need to provide compute resource isolation over all concurrently running GPU operations. Better
    }
 
   
%\item 
%\vspace{-2mm}
\Scut{
\subsection{Offloading Data Transfer to DMA}%\vspace{-2mm}
\knote{Do we need this subsection? We have this in both NetML and CloudNet papers. What aspect is new? Maybe better to just refer and say we use it. Especially the cluster related things are not likely to fit in this paper. We can just say we leverage the NetML capability. Aditya: Ok. I will just write we levarage approach from other papers.}
\update{Data transfer to GPU is often significant overhead for applications running in GPU. Current GPU runtimes require the data to be "pushed" to the GPU. First, the data has to be copied into a contiguous page-locked 'pinned' memory buffer, consuming CPU cycles, prior to a GPU runtime API call to initiate the transfer to GPU. Moving the data to GPU by CPU can limit throughput, with the CPU potentially becoming the bottleneck. \Scut{This is because copying and aggregating the data from packet payloads into a contiguous buffer on the CPU and then pushing the aggregated buffer to the GPU using the GPU runtime API consumes both CPU and memory cycles.}

We can avoid this extra copy by running a GPU kernel the uses the GPU's DMA engine to perform scatter-gather from host memory. Offloading the data transfer to GPU and have it "pull" data into GPU memory involves a relatively small amount of GPU processing, while reducing CPU cycles. In our system where we use the DPDK-based framework to receive network packets, we use NVIDIA's Unified Virtual Addressing (UVA)~\cite{schroeder2011peer} to initiate scatter-gather from packet payload to GPU. We pin the packet memory buffer pool (mbuf pool) and all incoming network packet data resides in the pinned memory region. Once we receives all the packets to execute a task, we launch a CUDA kernel to gather data from these packets into a GPU buffer similar to \cite{8806698}. We see the result of offloading the data transfer to DMA in Table.~\ref{tab:dma_offload_latency}. We see that the CPU cycles used in transferring the image while performing inference is an order of magnitude higher when copying data from packets to contiguous buffer and launching \textit{cudaMemcpy()} (CPU-Copy) API compared to the DMA-Offload. We can also see that the CPU cycles used in transferring the image while performing inference is an order of magnitude higher when copying data from packets to contiguous buffer and launching \textit{cudaMemcpy()} API compared to the DMA-Offload. The CPU load only gets higher with a larger number of images as the batch size increases.

We see the benefit of our approach when inferring a stream of images in a single and multi-GPU cluster. In Fig.~\ref{fig:single_gpu_inference}, the throughput of both CPU-Copy and DMA offloading increases as the request rate increases. The DMA-offloading's throughput is higher once the request rate is higher than 2000 images per second. Throughput with DMA offloading flattens out at about 4500 images/second as the single GPU becomes the bottleneck and cannot infer a higher rate of images. In contrast CPU-Copy approach has a much lower throughput as the CPU becomes bottleneck, thus, starving GPU of data. Similarly, with 8 GPUs we can have much higher inference throughput as seen in Fig.~\ref{fig:multi_gpu_inference}. With CPU-Copy data transfer, the inference throughput is limited to 3500 images/sec. But, with DMA offloading, we can process incoming requests up to 8000 images/sec. Therefore, GPU DMA is very benefical for inference of streaming data.

Other methods of transferring data from NIC to GPU such as GPUDirect also bypasses CPU. However, GPUDirect is only available in limited number of NICs and GPUDirect transfers the data directly to GPU. Unlike GPUDirect, our technique is applicable across all NICs.%, including the vast number of NICs that do not support GPUDirect. 
Moreover, using the CPU as an intermediary for determining when to transfer the data allows us to first selectively complete the network and security protocol processing, which are  more efficiently processed in the CPU~\cite{go2017apunet}. Therefore, while alternatives like GPUDirect exist for data transfer, we still consider the DMA-offload as necessary, since it can be deployed without requiring a specific NIC.
}

\begin{table}[]
    \centering
    \captionof{table}{Alexnet inference with different data transfer methods}
    \label{tab:dma_offload_latency}
    \vspace{-3mm}
   \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|}\hline
         Metric&CPU-Copy  & DMA-offload\\\hline
         CPU Cycles (Batch 1)&436878 &19083\\
         CPU Cycles (Batch 8)&3381260 &172632\\
         Inference Latency (Batch 1) & 3.25 ms &3.01 ms\\
         Inference Latency (Batch 8) &10.53 ms & 9.68 ms\\
         \textit{cudaMemcpy}/Data transfer kernel (b = 1) &77 $\mu$s & 108 $\mu$s\\
         %\vtop{\hbox{\strut \textit{cudaMemcpy} / Data transfer kernel (b = 1)}\hbox{\strut kernel runtime (Batch 1)}} &77 $\mu$s & 108 $\mu$s\\
         %\vtop{\hbox{\strut \textit{cudaMemcpy} / Data transfer }\hbox{\strut kernel runtime (Batch 8)}} &632 $\mu$s &880 $\mu$s \\\hline
          \textit{cudaMemcpy}/Data transfer kernel (b = 8)&632 $\mu$s &880 $\mu$s \\\hline
    \end{tabular}}
\end{table}

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
    \includegraphics[width=\linewidth]{figures/netml_high_data_rate/mobilenet_netml_vs_not_netml_single_gpu.pdf}
    \caption{One V100 GPU}
    \label{fig:single_gpu_inference}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
    \includegraphics[width=\linewidth]{figures/netml_high_data_rate/mobilenet_netml_vs_not_netml_multi_gpu.pdf}
    \caption{8 GPU T4 cluster}
    \label{fig:multi_gpu_inference}
    \end{subfigure}
    \caption{Alexnet CPU-Copy vs. DMA-offload throughput}
\end{figure}
}
\Scut{
GPU systems today have state-of-art physical memory with very high bandwidth (often more than 900 GB/s). This high bandwidth allows GPU to mask \knote{why do we need to talk about masking weak threads? Instead why not say we can take advantage of a lot of GPU threads accessing the memory simultaneously?} the weak GPU threads. To utilize this memory better, \knote{why not just say that typical operation is to get the data to the GPU memory and then allow them to work with the data in the GPU memory?} data related to GPU operations are required to be transferred to the GPU.}
\Scut{ Shorten REWRITE
Discrete GPUs are typically across the PCIe bus  requiring PCIe transactions to transfer data from CPU to GPU and vice-versa. Current GPU runtimes require the data to be "pushed" to the GPU. First, the data has to be copied into a contiguous page-locked 'pinned' memory buffer, consuming CPU cycles, prior to a CUDA API call to initiate the transfer to GPU. In a multi-GPU cluster that serves thousands of requests, this CPU overhead for data transfer to the GPU becomes crucial. Moving the data to GPU by CPU can limit throughput, with the CPU potentially becoming the bottleneck. This is because copying and aggregating the data from packet payloads into a contiguous buffer on the CPU and then pushing the aggregated buffer to the GPU using the GPU runtime API consumes both CPU and memory cycles.} %We show that CPU becomes the bottleneck due to data transfer workload as the incoming request/data rate increases. 

%\begin{table}[]
%\begin{figure}

\Scut{
\begin{minipage}{\linewidth}

\begin{minipage}[t!]{.45\linewidth}
    %\centering
    \flushleft
    %\vspace{-4mm}
    %\subfloat[Alexnet inference with different data transfer methods]{
    \captionof{table}{Alexnet inference with different data transfer methods}
    \label{tab:dma_offload_latency}
    \vspace{-3mm}
   \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|}\hline
         Metric&CPU-Copy  & DMA-offload\\\hline
         CPU Cycles (Batch 1)&436878 &19083\\
         CPU Cycles (Batch 8)&3381260 &172632\\
         Inference Latency (Batch 1) & 3.25 ms &3.01 ms\\
         Inference Latency (Batch 8) &10.53 ms & 9.68 ms\\
         \textit{cudaMemcpy}/Data transfer kernel (b = 1) &77 $\mu$s & 108 $\mu$s\\
         %\vtop{\hbox{\strut \textit{cudaMemcpy} / Data transfer kernel (b = 1)}\hbox{\strut kernel runtime (Batch 1)}} &77 $\mu$s & 108 $\mu$s\\
         %\vtop{\hbox{\strut \textit{cudaMemcpy} / Data transfer }\hbox{\strut kernel runtime (Batch 8)}} &632 $\mu$s &880 $\mu$s \\\hline
          \textit{cudaMemcpy}/Data transfer kernel (b = 8)&632 $\mu$s &880 $\mu$s \\\hline
    \end{tabular}}
    %\vspace{-4mm}
   %\vspace{-4mm}
   \end{minipage}%
   
   \begin{minipage}[t!]{.25\linewidth}
   %\subfloat[Single V100 GPU inference]{
    \includegraphics[width=\linewidth]{figures/netml_high_data_rate/mobilenet_netml_vs_not_netml_single_gpu.pdf}
    %\caption{Caption}
    \captionof{figure}{One V100 GPU}
    \label{fig:single_gpu_inference}%}
    \end{minipage}%
    \begin{minipage}[t!]{.25\linewidth}
    %\subfloat[8 GPU T4 cluster inference]{
    \includegraphics[width=\linewidth]{figures/netml_high_data_rate/mobilenet_netml_vs_not_netml_multi_gpu.pdf}
    \label{fig:multi_gpu_inference}%}
    \vspace{-3mm}
    \captionof{figure}{8 GPU T4 cluster}
    \end{minipage}
    %\subfloat[Power consumption on smaller image 224x224. The trend is similar as left figure but not clearly visible.]{\includegraphics[width=.5\linewidth]{figures/hotnets_plot/power_statistics_all.pdf}}
   %\caption{CPU-copy vs. DMA-offload Mobilenet throughputs (high request rate) }
   \end{minipage}
  %\end{figure}
  }
  
\Scut{
  \begin{figure}
    \centering
    \subfloat[Single V100 GPU inference]{
    \includegraphics[width=.33\linewidth]{figures/netml_high_data_rate/mobilenet_netml_vs_not_netml_single_gpu.pdf}
    %\caption{Caption}
    \label{fig:single_gpu_inference}}
    \subfloat[8 GPU T4 cluster inference]{\includegraphics[width=.33\linewidth]{figures/netml_high_data_rate/mobilenet_netml_vs_not_netml_multi_gpu.pdf}
    \label{fig:multi_gpu_inference}}
    \vspace{-2mm}
    %\subfloat[Power consumption on smaller image 224x224. The trend is similar as left figure but not clearly visible.]{\includegraphics[width=.5\linewidth]{figures/hotnets_plot/power_statistics_all.pdf}}
   \caption{CPU-copy vs. DMA-offload Mobilenet throughputs (high request rate) }%\sknote{Can we fix the figure number for these plots?}.
   \vspace{-6mm}
\end{figure}
}
%\end{table}
%Copying the payload from each packet separately to the GPU (using CUDA API calls such as \textit{cudaMemcpy}) is very expensive. A better method is to first copy and aggregate the data from packet payloads into a contiguous buffer and then DMA the aggregated buffer to the GPU. 
%However, even this method taxes both CPU and memory to copy and store data in the contiguous buffer.
%However, this method consumes additional memory and lot of CPU cycles to copy the data from packets to a contiguous buffer. 
\Scut{We can avoid this extra copy by running a GPU kernel the uses the GPU's DMA engine to perform scatter-gather from host memory. Offloading the data transfer to GPU and have it "pull" data into GPU memory involves a relatively small amount of GPU processing, while reducing CPU cycles.  % taking off workload from CPU.
%%%%%%%%%%%%% non required writing
\Scut{
 Alternative for data transfer include a NIC to GPU transfer using GPUDirect.%, and host memory to GPU transfer using MMIO. 
 However, GPUDirect places all ingress packets into GPU memory and the GPU kernels have to perform packet processing. But this has many limitations such as inefficient packet processing in GPU~\cite{vasiliadis2014gaspp}. \Scut{Alternately, MMIO approaches require the CPU to copy the data into a specific pinned memory. The data has to be then moved into GPU using DMA. Thus, this approach incurs high CPU overhead.} Using the approach of ~\cite{dhakal2019netml},
%the zero-copy scatter-gather approach \Scut{from ~\cite{Anonymous}},
we only transfer \Scut{ML processing} relevant data for ML processing to the GPU, with packet processing in the CPU. This avoids CPU copies, thus relieving the CPU bottleneck at high data rates.}
%\trackchange{%Typical MMIO approaches require CPU copies to place data in specific pinned memory, then moved into GPU using DMA. GSLICE avoids this using zero-copy DMA scatter-gather of packet-payload to GPU.}
\Scut{\newline\noindent\textbf{Data transfer to GPU}:
DPDK enables the ethernet driver to transfer packets to shared hugepage buffers that can be accessed with zero-copy. %Those packets are accessible with zero-copy to all the DPDK applications that have mapped to the shared memory region. 
Copying the payload from each packet separately to the GPU (using CUDA API calls such as \textit{cudaMemcpy}) is very expensive. A better method is to first copy and aggregate the data from packet payloads into a contiguous buffer and then DMA the aggregated buffer to the GPU. 
However, even this method taxes both CPU and memory to copy and store data in the contiguous buffer.
%However, this method consumes additional memory and lot of CPU cycles to copy the data from packets to a contiguous buffer. 
We avoid this extra copy by running a GPU kernel which employs
%employing 
the GPU's DMA engine to perform scatter-gather across host memory. This }
%%%%%%%%%%%%%%%%%%% Edit from below %%%%%%%%
%To transfer network packet payload data to the GPU, 
We use NVIDIA's Unified Virtual Addressing (UVA)~\cite{schroeder2011peer}, %. It allows a CUDA kernel running in the GPU to directly use and access the host's virtual memory address. %When a GPU thread encounters a host side address, it stalls while the GPU's DMA engine DMA the data and fetches it into GPU memory. 
%However, UVA 
that requires the host-side data to be a page-locked (pinned) memory area. %In \netml method, when a DPDK based ML application creates a GPU context, 
In our system where we use the DPDK-based framework to receive network packets, the packet memory buffer pool (mbuf pool) is already pinned and
%Hence, 
%we pin DPDK's  \Scut{during IF initialization} to ensure that 
all incoming network packet data resides in the pinned memory region. 
\Scut{We use \texttt{rte\_eal\_get\_configuration()} of the DPDK API to obtain the virtual address of the mbuf pools and register these addresses with the GPU using \texttt{cudaHostRegister()} CUDA API. We profiled the time to pin 1GB memory to be \textasciitilde 20ms.}
Once we %on the host side 
receives all the packets to execute a task, we launch a CUDA kernel %(Algorithm \ref{Algo:Data_Transfer_kernel}) 
to gather data from these packets into a GPU buffer similar to \cite{8806698}.
We see the result of offloading the data transfer to  DMA in Table.~\ref{tab:dma_offload_latency}. We see that the CPU cycles used in transferring the image while performing inference is an order of magnitude higher when copying data from packets to contiguous buffer and launching \textit{cudaMemcpy()} API compared to the DMA-Offload. The CPU load only gets higher with a larger number of images as the batch size increases. %Offloading the DMA to GPU has much lower CPU load. 
DMA offloading also reduces the overall inference latency. While, DMA offloading reduces CPU-load, the GPU has to run a data transfer kernel to induce GPU DMA engine to initiate DMA. This kernel has a small GPU overhead as we launch one GPU thread per network packet, thereby using less than 600 GPU threads for initiating the transfer of 1 image. We see from the Table~\ref{tab:dma_offload_latency} that the data transfer kernel runs for about 900 $\mu$s for transferring  8 images. This time is slightly longer than the time CUDA memcpy takes to transfer 8 images to GPU. But, this CUDA memcpy first requires the CPU to copy data to contiguous buffer first before transferring data to GPU which consumes time. On the other hand, the GPU DMA can perform th before launching the CUDA kernel operations that act on the data. Moreover, any data corruption would basically stall both the CPU and GPU processing until the consistency of data is guaranteed. Further, with streaming data, this issue can greatly affect the performance when operating in large batch sizes as any loss or corruption of a single packet would engender the entire batch of DMAed data to be unusable. 
However, with our DMA-offload technique, these issues do not arise, as the CPU thread is involved in launching the data transfer kernel and the subsequent CUDA kernels, it can do so only after ensuring the data consistency and also choose to skip the transfer of malformed data without affecting the batching. More importantly, unlike GPUDirect, our technique is applicable across all NICs.%, including the vast number of NICs that do not support GPUDirect. 
 Moreover, using the CPU as an intermediary for determining when to transfer the data allows us to first selectively complete the network and security protocol processing, which are  more efficiently processed in the CPU~\cite{go2017apunet}. Therefore, while alternatives like GPUDirect exist for data transfer, we still consider the DMA-offload as necessary, since it can be deployed without requiring a specific NIC.


An alternative approach in~\cite{rhu2018compressing} %uses zero-compression \knote{what is zero compression? Why not just say compression?} to 
compresses the data before transferring from CPU to GPU, to significantly improve data transfer throughput. However, this requires the original uncompressed data to be in a contiguous memory location. Similarly, the compressed data has to be written to another contiguous memory location before the DMA to GPU. Both of these operations consume significant amount of CPU cycles, especially when data is streaming in from the network and is scattered across multiple memory locations.   
%While, the data compression can help increase throughput, it requires the uncompressed data to be in  as well as writes the compressed data into a different contiguous memory before DMA to GPU. In a system where data is being received from network packets, the data is not aggregated but is scattered in different memory location. 
Thus, our approach of using a GPU resident DMA avoids these overheads and does not require data to be in contiguous location.


%We conducted an experiment by gradually increasing the number of requests (image) sent to an Alexnet IF. We then process the received request with a batch of 32 using the GPU. We show the improved throughput with the zero-copy GPU transfer versus the copy and transfer to the GPU method in the Figure below.

%The effect of high CPU cycles used for copying and transferring data to GPU can be seen when receiving a huge 
We see the benefit of our approach when inferring a stream of images in a single and multi-GPU cluster. In Fig.~\ref{fig:single_gpu_inference}, we see that the throughput of inference of Alexnet for both CPU-Copy and DMA offloading increases as the request rate increases. The DMA-offloading's throughput is higher once the request rate is higher than 2000 images per second. Throughput with DMA offloading flattens out at about 4500 images/second as the single GPU becomes the bottleneck and cannot infer a higher rate of images. In contrast CPU-Copy approach has a much lower throughput as the CPU becomes bottleneck, thus, starving GPU of data. We present a similar experiment in the multi-GPU cluster in Fig.~\ref{fig:single_gpu_inference}. With 8 GPUs we can have much higher inference throughput. With CPU-Copy data transfer, the inference throughput is limited to 3500 images/sec. But, with DMA offloading, we can  process incoming requests up to 8000 images/sec. Offloading the data transfer to GPU DMA is very beneficial for inference of streaming data at high bandwidths.
}

%\end{itemize}

\vspace{-1mm}\subsection{Improved GPU resource management}\vspace{-1mm}
\update{The current CUDA MPS ver. R450~\cite{nvidiamps2019} %\sknote{Aditya, please help get the right version and citation for our usage} 
strictly limits the configuration of the GPU resource partition (GPU\%) to a one-time (static) allocation that is set prior to the GPU initialization of the application. This limitation poses a major challenge, as any GPU resource readjustment would require us to spin up a new CPU process with an updated GPU\%, which can take several seconds (depending on the ML framework initialization).}\Scut{This necessitates that having a set of operating system level primitives and design principles that can provide loss-free and interruption-free execution of the applications while %ensuring the progress of the GPU tasks, 
at the same time providing dynamic updates %to the scale 
of the mapped CPU and GPU resources.
We introduce a %number of %additional CUDA %/CuDNN 
rich set of CPU-GPU primitives and DNN framework level enhancements to dynamically adapt the GPU resources. Our technique facilitates low-overhead periodic application level monitoring and change of GPU\% with negligible downtime. } 
%without lowering DNN model's performance with %improve management of GPU resources and provide efficient, controlled, multiplexing of the GPU processing across multiple DNN models.
\Scut{
\begin{itemize}
    \item \textbf{Partitioning of Resources:} We have explicit ability to partition GPU for each running application. The GPU resource should be able to partitioned into parts and provided to running applications. This partitioning should be based on knee of the application.
    \item \textbf{Resize of Resource partition/Reduce Fragmentation:} The GPU resources provided to an application might not be enough for increased request count or increased batch size. Therefore, we need a system that will quickly adjust the resource partition of all applications running in GPU. However, changing partition in GPU is not easy and takes a long time. There are few ways to lower the load time (parameter sharing, CPU side pre-loading \etc). However, one should be careful on not losing any work while resizing, therefore, the overlapping of getting new Model setup and old model continue to function should exist. Furthermore, multiplexing lot of application will cause the allocated resource to be fragmented. Therefore, we need primitives to reduce resource fragmentation.
    \item \textbf{Overlap of Execution:} While resizing the GPU partition or correcting fragmentation we might need to change the original IF's resource allocation or consolidate multiple IFs into a single one. We have to make sure that there is an overlap of execution, such that the application that is processing inferences should keep processing without losing "effective work" until the new instance with "proper" resource allocation is ready. The scenario for an overlap might be: Original IF wants to finish processing requests it already has put into GPU, execution of current round of inference finishes for all concurrently run IFs, have to wait till secondary IF is ready, then we have to co-ordinate the overlap.
    \item \textbf{GPU Utilization:} GPU utilization metrics provided by NVIDIA do not show the true picture of utilization. We can infer GPU being utilized by looking at amount of power GPU is using. 
\end{itemize}
}




\Scut{
\begin{figure}[H]
\vspace{-6mm}
    \begin{center}
    \includegraphics[width=.33\linewidth]{figures/memory_throughput/memory_throughput.pdf}
    \caption{Global Memory Load Throughput of VGG-19 kernels while multiplexing }
    \label{fig:vgg-19-kernels-throughput}
    \end{center}
    \vspace{-6mm}
\end{figure}
}



\subsubsection{Dynamic adaptation of GPU resources}
%\newline\noindent\textbf{Dynamic adaptation of GPU resources}: %{Dynamic Resizing}
The GPU resources provided to an application might need to change over time due to the variations in the workload, \ie the change in arrival rate of the tasks (especially with streaming data), or the variations in the number of concurrently executing applications either due to the addition of new applications or termination of currently executing applications. Further, when an application terminates, it is necessary 
%we need 
to reclaim and redistribute the GPU resources among the active applications to avoid any resource fragmentation and under-utilization of the GPU. 
Therefore, %to address such dynamic workload variations, 
we need a system that can quickly and dynamically adjust the GPU resource partition of all the active applications. \Scut{Overall, addressing these aspects demands a rich set of CPU-GPU primitives and a closed-loop framework that can facilitate lightweight, low-overhead, periodic application level workload monitoring and change detection support, an optimization framework to provision and configure the right amount of GPU resources and task batching support for the 
%concurrently running 
applications.}

\Scut{\knote{although this para and the next are not strictly duplicating, I think it would be better to comment out this para, and just focus on the next para on mechanism. If there is space, we can keep it.}
However, dynamically adapting the GPU resource profile across all the active applications is non-trivial. 
First, we need the ability to monitor the request rate and service rate for each of the inference applications and then detect the overload or under-load condition and correspondingly adjust the CPU/GPU resources. 
Second, we need to ensure that the resource readjustment for an application is loss-free, does not entail any SLO violations, and does not have an adverse impact on inference latency. Finally, we also need to make sure that the overheads for performing such resource re-allocations are not excessive, so as to undermine the benefit of performing the resource reallocation. \knote{remove up to here.}
}
\Scut{
Overall, addressing these aspects demands a rich set of CPU-GPU primitives and a closed-loop framework that can facilitate lightweight, low-overhead, periodic application level workload monitoring and change detection support, an optimization framework to provision and configure the right amount of GPU resources and task batching support for the 
%concurrently running 
applications. More importantly, we need an agile and rapid CPU and GPU resource re-provisioning scheme to ensure loss-free and interruption free inference processing.
%an agile and swift switchover capability that can ensure loss-free and interruption-free CPU and GPU resoruce reprovisioning.
Accordingly, we develop a light-weight Orchestration framework and a library that can be easily plugged-in with the inference applications.}
%\vspace{-4mm}

\newline\noindent\textbf{Monitoring and Detection}:
Our library facilitates tracking the arrival rate and service rate of inference tasks and achieved SLO for each application using simple counters and a lightweight \textit{DPDK timer} interface. Using these parameters and the configured GPU\% and batch size, the library then determines whether the application is overloaded or is under-utilizing the GPU resources, and correspondingly triggers  reconfiguration of the resource allocation. 
\Scut{The pseudocode~\ref{Algo:GPU_tuning} is used to determine the overload or under-load scenario for an application and accordingly proposes for the new scale factor for the GPU resources.}
\Scut{
\begin{algorithm}[H]
%\LinesNumberedHidden
%\LinesNumbered
%\SetAlgoLined
%\DontPrintSemicolon
\KwIn{$\mathit{currentGPU\%,SLO,arrivalRate}$}%\tcp*{All CUDA Streams}}
\SetKwFunction{FMain}{ComputeNewGPU\%}
\SetKwProg{Fn}{Function}{:}{\KwRet{newGPU\%}}
\Fn{\FMain{}}{
avgL$\gets$LatencyHistogram.EWMA()\\
avgT$\gets$ThroughputHistogram.EWMA()\\
residualL$\gets$SLO $-$ avgL\\
residualT$\gets$avgT $-$ arrivalRate\\
diffL\%$\gets\frac{residualL\times100}{SLO}$\\
diffT\%$\gets\frac{residualT\times100}{arrivalRate}$\\
\If{(diffL\% $<$ threshold) $\&\&$
\mbox{}\phantom{\textbf{if}} (diffT\% $<$ threshold)}{
\KwRet{currentGPU\%}
}
\vspace{-2mm}
changeFactor $\gets$MAX$\left(\frac{\mathit{abs(residualL)}}{\mathit{avgL}},\frac{\mathit{abs(residualT)}}{\mathit{avgT}} \right)$\\
changeGPU\% $\gets$ currentGPU\% $\times$ changeFactor\\
\If{(residualL $<$ 0) $\|$ (residualT$<$0)}{
    newGPU\% $\gets$ currentGPU\% $+$ changeGPU\%
}
\If{(residualL $>$ 0) $\&\&$ (residualT$>$0)}{
    newGPU\% $\gets$ currentGPU\% $-$ changeGPU\%
}
}
\caption{Load Monitoring, Detection and GPU Resource Allocation Algorithm}
\label{Algo:GPU_tuning}
\vspace{-1mm}
\end{algorithm}%\vspace{-3mm}
}
%\vspace{-2mm}

\Scut{
\begin{algorithm}[!htbp]
%\vspace{-1mm}
\caption{Active to Standby Switchover}
\label{algo:activetostandby}
\begin{algorithmic}[1]
\Procedure{\texttt{ResourceReadjust}$(\mathit{standby,NewGPU\%})$}{}
%\STATE\hspace{\algorithmicindent} $<\mathit{standbyDNN, GPUFlag}> = 1$
\State $<\mathit{standby, GPUExFlag}> = 0$ \Comment{No GPU Execution}
\State $<\mathit{standby, GPU\%}> = NewGPU\%$\Comment{GPU access}
\State sendMessage$(\mathit{standby,} \texttt{GetReady})$
\EndProcedure
\State
\Statex{{\bf Event:} \texttt{ReceiveMessage}}
\If{msg = $<\mathit{standby,} \texttt{modelLoaded}>$}
    \State sendMessage$(\mathit{active,} \texttt{CompleteWork})$
\EndIf
    \If{msg$ =<\mathit{active,\texttt{workCompleted}}>$}
    \State $<\mathit{active, GPUExFlag} > = 0$ \Comment{Stop GPU execution}
    \State $<\mathit{standby, GPUExFlag} > = 1$ %\Comment{Allow GPU execution}
    \State wakeUp$\mathit{(standby})$ \Comment{Trigger Standby Wakeup}
    \State shutdown$(\mathit{active})$
    \State $\mathit{active \gets standby}$ \Comment{Standby is new Active}
    \State startNewStandbyInstance$()$
\EndIf
\Statex{{\bf End Event}}
\end{algorithmic}
%\vspace{-4mm}
\end{algorithm}%\vspace{-4mm}
}


\Scut{
\begin{algorithm}[H]
\caption{Active to Standby Takeover: Active DNN}
\label{algo:activeDNN}
\begin{algorithmic}[1]
\Statex{{\bf Event:} \texttt{ReceiveMessage}}
\If{msg = $<\mathit{Manager,} \texttt{CompleteWork}>$}
\While{$\mathit{DNNInferencePending} > 0$}
\State wait() \Comment{Waits for inference results}
\EndWhile{}
\State sendMessage$(\mathit{Manager,} \texttt{workCompleted})$
\State cleanup() \Comment{Wait for Shutdown}
\EndIf
\Statex{{\bf End Event}}
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[H]
\caption{Active to Standby Takeover: Standby DNN}
\label{algo:standbyDNN}
\begin{algorithmic}[1]
\Statex{{\bf Event:} \texttt{ReceiveMessage}}
\If{msg = $<\mathit{Manager,} \texttt{GetReady}>$}
\If{$GPUFlag == 1$}
\State setEnvVar($\mathit{newGPU\%}$)
\State LoadModel() \Comment{Load DNN model in GPU}
\State sendMessage$(\mathit{Manager,} \texttt{modelLoaded})$
\State sleep() \Comment{Sleep till woken by the manager}
\EndIf
\EndIf
\Statex{{\bf End Event}}
\Statex{{\bf Event:} \texttt{Wakeup}}
\State pendingInference() \Comment{Finish pending requests from active}
\State inferRequests() \Comment{Infer new requests}
\Statex{{\bf End Event}}
\end{algorithmic}
\end{algorithm}

}%\vspace{-4mm}
\Scut{
\newline\noindent\textbf{Resource Allocation}: We develop a lightweight optimization problem that considers the current application heterogeneity, workload demands and SLO parameters to provide the right GPU resource allocation and batch size for all the concurrently running applications (more details in \S~\ref{sec:efficient_batch_size}).}
%\knote{we need to put the right label for the reference.} %\ref{sec:optimization}). \knote{are you using this as a precursor to saying how you will then have a software primitive to say that the application or something will ask the library for this allocation?} \sknote{yes.}
\Scut{Hence, we propose a lightweight optimization problem that considers the current application heterogeneity, workload demands and SLO parameters to provide the right GPU resource allocation and the batch size for all the applications.}
%\knote{why are we talking about the optimization here? We should be focused on the software primitive we want to use to allow for the adaptation, and leave the discussion for the need to set the right value and how that right value is determined to the optimization section. So, move this last sentence to the opt. section.}\sknote{Okay, I just wanted to highlight the need for Optimization framework here. It can be commented or moved to optimization section too.}
\newline\noindent\textbf{Resource readjustment}:\Scut{ The current CUDA MPS ver. R450~\cite{nvidiamps2019} %\sknote{Aditya, please help get the right version and citation for our usage} 
strictly limits the configuration of the GPU resource partition (GPU\%) to a one-time (static) allocation that is set prior to the GPU initialization of the application. This limitation poses a major challenge, as any GPU resource readjustment would require us to spin up a new CPU process with an updated GPU\%, which can take several seconds (depending on the ML framework initialization). This necessitates that having a set of operating system level primitives and design principles that can provide loss-free and interruption-free execution of the applications while %ensuring the progress of the GPU tasks, 
at the same time providing dynamic updates %to the scale 
of the mapped CPU and GPU resources. }
%Thus to ensure loss-free and interruption free progress of the GPU tasks, we devise application replicas (several, or at-least two processes on the CPU with active(1):standby(n) mode)
For this, we create application replicas (several, or at-least two processes on the CPU with active(1):standby(n) mode) and employ a deferred GPU initialization for the replica (standby). Also, we incorporate a handover scheme such that the application processing the inference (active) continues to make progress until the new instance (standby), with its updated resource allocation, is ready to takeover. 
%\anote{Put in sentence saying "when loading a new model, the active model's throughput does not decrease as the compute resources are not affected.}

We build a state model for the Inference application (active and standby) % such that the switchover is handled in a seamless and loss-free manner. 
as shown in the Algorithm~\ref{algo:activetostandby}, %fig~\cite{fig:switchover}, 
that describes the necessary primitives we developed for providing seamless and loss-free switchover. The orchestration framework makes use of the event-action control loop and asynchronous message notifications to the active and standby processes.  
Lines 1:3 indicate the state maintained in the library to initiate the switchover. Here, the notification is sent to the standby DNN process to start preparing the initialization phase by updating the desired %appropriate 
\textit{NewGPU\%} (between 1 to 100). We also use a boolean flag,  \textit{GPUExFlag}, to control the status of inference operation (dormant (0), running (1)).
%of the standby is transitioned from 0 to 1 indicating that it can now start performing the inference operations
First the \textit{GPUExFlag} is kept 0, but the \textit{NewGPU\%} is transitioned from 0 to a desired value indicating that 
it can now start initializing the GPU and configure the GPU resources with the input \textit{NewGPU\%}.
%\knote{it is confusing whether the NewGPU\% is a boolean or a value of the GPU\%??? Please clarify}
Lines 7:8 Once the standby DNN process notifies the completion of initialization phase, the Orchestrator next notifies the current primary (Active) DNN to complete its current set of inference tasks and stop processing any further inference operations. 
Lines 10:16 After the primary instance notifies back its completion status, the \textit{GPUExFlag} of the standby is transitioned from 0 to 1 indicating that it can now start performing the inference operations. The standby is  transitioned to being the new active GPU task, while the earlier active process is terminated and a new standby is created subsequently. 
This mode switching ensures loss-free and interruption-free inference processing for the application. %providing a momentary overlapped execution of inference tasks among the active and standby instances.
%\knote{Is there a succinct way to describe the software primitive we need for achieving this?}\sknote{I have updated it, bur find it hard to cut down.}\knote{I mean that we need to provide what the essential software primitive we need beyond what is there in the previous point about 'controlled sharing' - I am saying about 'dynamic adaptation'}

\newline\noindent\textbf{Memory impact during Spatial Sharing}: Previous work, such as~\cite{jog2015anatomy}, has observed that concurrently running applications can interfere with each other in the GPU memory subsystem, resulting in higher latency for kernel execution. We analyzed the memory contention during inference using multiple DNNs, with controlled spatial sharing, by increasing the number of concurrent DNN models. We look at the \textit{global\_load\_throughput} which shows the memory bandwidth obtained by kernels while loading data from GPU main memory for 10 different VGG-19 kernels in Fig.~\ref{fig:vgg-19-kernels-throughput}. We can see that as the number of concurrent processes (multiplexed DNN applications) increases %\knote{is this X-axis, number of concurrent processes? If so, why not use the same terms in the legend in the graph and the writing?}
, the global memory load throughput decrease is marginal for most kernels (less than 5\%), and only for kernel 5 it reduces a little more than 20\% while going from 1 to 5 concurrently running DNNs. %This reduced memory throughput is due to contention caused by multiple DNN kernels running concurrently. 
While we do observe some memory contention, the DNN models we have studied do not appear to be memory bandwidth constrained. 
%Furthermore, spatial multiplexing of DNNs does not suffer because of the small reduction in the memory throughput, as we do not see a corresponding degradation in inference\Scut{task completion time} latency even when multiplexing 10 different DNN processes in the GPU. 
Overall the benefit we derive from controlled spatial sharing of DNNs far outweighs any concerns regarding memory bandwidth contention within the GPU.
\subsection{Other Runtime Primitives}
\newline\noindent\textbf{GPU-DMA for network data}: Transferring streaming data arriving from network to GPU is expensive in terms of CPU. CPU have to copy the data from packet payload and again transfer data using GPU runtime APIs causing the CPU to be bottleneck in a system processing huge amount of streaming data. We utilize GPU-DMA to transfer data with low CPU overhead and provide high inference throughput as described in ~\cite{dhakal2019netml}. \newline\noindent\textbf{Parameter sharing during Resource readjustment}: When adjusting the resources, the replica (standby) instance has to load its model into GPU with an updated GPU\% specified, while the active process still has to infer incoming requests. We have observed that the loading of another model does consume additional memory temporarily, but the reduction in the total memory footprint due to parameter sharing, \ie reusing the model parameters of original model to compensates for this increase as described in~\cite{GSLICE}. Moreover, it does not have any effect on latency and throughput of the currently running active model. % even though the standby instance consumes additional memory temporarily, the reduction in the total memory footprint due to parameter sharing compensates for this increase.
%\anote{I am trying to putting a nvprof profile to show shadow loading. }
%\knote{but memory is used up. you have to say that! Does this next sentence help for that?: 
%{yes!.}}

\Scut{
%The GPU resources provided to an application might not be enough for increased request count or increased batch size.
%However, changing partition in GPU is not easy and takes a long time. %There are few ways to lower the load time (parameter sharing, CPU side pre-loading \etc). However, one should be careful on not losing any work while resizing, therefore, the overlapping of getting new Model setup and old model continue to function should exist.
%Furthermore, multiplexing lot of applications will cause the allocated resource to be fragmented. Therefore, we need primitives to reduce resource fragmentation.While resizing the GPU partition or correcting fragmentation we might need to change the original IF's resource allocation or consolidate multiple IFs into a single one.
%We have to make sure that there is an overlap of execution, such that the application that is processing inferences should keep processing without losing "effective work" until the new instance with "proper" resource allocation is ready. The scenario for an overlap might be: Original IF wants to finish processing requests it already has put into GPU, execution of current round of inference finishes for all concurrently run IFs, have to wait till secondary IF is ready, then we have to co-ordinate the overlap.
}

\Scut{\textbf{Maximizing the GPU Utilization}:
%\textbf{GPU Utilization: Measurement and Maximization}:
GPU utilization metrics provided by NVIDIA do not show the true picture of utilization. We can infer GPU being utilized by looking at amount of power GPU is using. 
\knote{I am not sure that we want to use this to justify using power measurement as a stand-in for the buggy GPU util. measurement of nVIDIA. I'd rather not get into that, because people can say that is not reliable - we don't know how to prove that is correct. In fact, I suggest that we do not get into the problems of measurement, because we don't know how to do it correctly either.}\sknote{Okay. We can avoid mentioning about GPU Utilization measurement issues. But to support our claim of maximizing the GPU utilization, we can try to utilize Power measurement as means of efficient utilization and not mention anything more on this.}
\anote{Shall we try to measure FLOPS over long interval. We know how much computation each DNN takes (Theoretically) and we see the time it takes to execute them. Let's pick 5 second interval, and basically see how much FLOPS we were able to obtain by various sharing methods by counting how much inference was done. I see problem being we might lose out to Default MPS here as it might be having higher FLOPS and needing to fix batch size as higher batch size produce higher FLOPS for each model regardless of GPU sharing.}
}
%==================================================================
\Scut{
\subsection{Inference in Multi-GPU Cluster}
\begin{itemize}
    \item Multi-GPU inference necessary for higher throughput
    \item Higher throughput means more incoming data. Data movement can be problem
    \item Multi-GPU plus spatial sharing means, even same DNN might instances with unequal GPU resource. Therefore, we need load balancing among those DNNs.
\end{itemize}
Multi-GPU cluster is often employed to lower the training time for DNN models. Various distributed training algorithm exist to use multi-GPU cluster. %While training in multiple-GPUs frequently require gradient transfer across GPU to synchronize the gradients, the DNN model for inference usually resides in a single GPU. therefore, inference using multiple GPU usually helps increase the throughput of inference by distributing the inference load across multiple GPUs. 
Multiple GPU cluster provide a medium to horizontally scale DNN to process more requests by starting a new instance of same DNN in different GPU. However, with spatial sharing of a GPU with fixed GPU\% it is possible to run multiple instance of same DNN model with different amount of GPU resources. With unequal amount of GPU resources it becomes necessary to load balance between the two instances of the DNN models. 
%=================================================================
}
%==================================================================
%\vspace{-4mm}
\Scut{
\noindent\newline\textbf{Cluster-Wide GPU Multiplexing}: 
\knote{do we want to start with this experiment when all of our work is on a single GPU? Maybe we want to take it out of here and possibly use it in the future. Don't put in cluster-wide anything here, as it will confuse the reader. AD: I will cut it out.We will exapand on the multiplexing experiment Fig 15 (a) with temporal and spatio-temporal options.}
We ran an experiment with 5 DNN application instances on 3 of the GPUs (we were limited by network link bandwidth of 40 Gbps). %: 2 instances of ResNet-50, 2 instances of Mobilenet, and 1 instance of VGG-19,  
For the `default MPS (M)' and 'Fixed batch (FB) cases, our setup includes two instances each of Mobilenet on one GPU, and two instances of ResNet-50 on another GPU and single instance of VGG-19 on a third GPU, and the batch size is set to 1 in the `default MPS' and to 8 for the 'Fixed Batch' case respectively. 
For CSS case, we multiplexed one instance of ResNet-50 with 70\% of GPU and Mobilenet  with remaining 30\% (close to the percentages obtained from the optimization above) of the GPU. We instantiate the same setup on two different GPUs. Since VGG-19 is compute heavy, we gave an entire instance of GPU (with its 'knee' at 100\%). 
CSS uses self-learning adaptive batching as described in~\cite{GSLICE}, ensuring latency remains below the specified SLO. In CSS, we also implement offloading data movement to the GPU DMA, and the task completion notification.
In all the cases we used the same workload (input traffic using 40Gbps link). We compute the throughput achieved by the system, with a nominal SLO of 50 ms. Table~\ref{tab:css_all_together} shows the results of `default MPS (M)', `default MPS with Fixed batch (FB)' and `CSS' modes.
\looseness-1
\Scut{
\begin{table}[h]
\vspace{-4mm}
    \centering
    \caption{Avg. Throughput \& Latency in 3 GPU cluster}
    \vspace{-3mm}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}\hline
         Model&\multicolumn{2}{|c|}{Default MPS}  & \multicolumn{2}{|C|}{CSS}   \\\hline
         & Latency (ms) & Throughput(Ips) & Latency & Throughput\\\hline
         Mobilenet&5.27&1702&5.23&1708\\
         ResNet-50&37.88&503&24.83&713\\
         VGG-19&24.80&40&24.80&40\\\hline
    \end{tabular}}
    \label{tab:css_all_together}
    \vspace{-2mm}
\end{table}
}
With CSS, we achieve much higher throughput %when we multiplex each GPU with two different models 
compared to `M' and `FB' cases. %, thus showing the effectiveness of CSS in improving GPU utilization. 
ResNet-50 sees almost a {\bf 40\%}  throughput improvement over `FB', without sacrificing the performance for other models. CSS has the same average latency ($\sim$25 ms) for Mobilenet and VGG-19. Further, CSS has much better latency for Resnet-50, while `M' and `FB' show higher latency due to interference.\looseness-1 
}

==> sections/design.tex <==
\section{System Design and Architecture}
\subsection{GPU Cluster Management}




\iffalse
Paragraph: Describe current architecture. However, focus on Orchestrator which will be performing autoscaling, i.e. starting new instances. Figure of architecture.

\subsection{DPDK based NF environment}
Describe OpenNetVM architecture and how any new NF can be added and removed. Brief description on how the traffic is load balanced to multiple NF of same DNN. 

\subsection{Orchestrator}
Orchestrator is an important component for adding and removing compute nodes. Describe the functionality of Orchestrator. eg. it accepts message by ZMSQ library and then creates new node by forking existing program and loading CPU/GPU options provided by Manager.

\subsection{Autoscaling Algorithm}
An algorithm that we will use to find out how many new nodes we will create and nodes we will destroy. Eg. in our experiments we saw that after a certain point, adding more nodes did not help with throughput. Eg. for ResNet-50, 2 20\% Node do not perform better than 1 40\% node. Therefore, we consult a pre-computed table before increasing or decreasing the number of nodes.

Following things to consider:
\begin{itemize}
    \item The incoming rate for each IF.
\item Batch size: Should there be a fixed batch size? 
\item SLO
\end{itemize}{}
\setalgorithmicfont{\small}
\begin{algorithm}
\caption{Weighted Max-Min algorithm for $N$ IFs}
\begin{algorithmic}[1]
\Procedure{WMAX-MIN}{$knee[N],maxGPU\%$}
\State {$remGPU$ $\gets$ $maxGPU\%$}
\State {$retGPU[N]$ $\gets$ $0$}
\State {$totDemand$ $\gets$ $\sum_{k=1}^{N}knee[k]$}
\For{$i \gets 1$ to $N$}\Comment{Fulfill Lowest Demand First}
\If{$remGPU$ $\geq$ $knee[i]$}
\State{$retGPU[i]$ $\gets$ $knee[i]$}
\State{$remGPU$ $\gets$ $remGPU - knee[i]$}
\ElsIf{$remGPU$ $>$ $0$}
\State{$retGPU[i]$ $\gets$ $remGPU$}
\State{$remGPU$ $\gets$ $0$}
\EndIf
\EndFor
\If{$remGPU$ $\geq$ $0$}
\Comment{Proportionally divide rest GPU\%}
\For{$j \gets 1$ to $N$}
\State{$retGPU[j]$$+=$$\frac{knee[j] }{totDemand}$ $\times remGPU$   }

\EndFor
\EndIf
\EndProcedure
\end{algorithmic}

\end{algorithm}

==> sections/evaluation.tex <==
\section{Evaluation}
\subsection{Experiment 1: }























\Scut{
Preliminary result:\\
We ran an experiment with resnet50 model in 2 Streams, one with priority of 1 and another with priority of 2 \knote{simultaneously???, AD: yes}.
The lower priority number means higher stream priority. 
The mean latency for priority of 2 was 17.234 ms for inferring 1 image.
The mean latency for priority of 1 was 8.809 ms for inferring 1 image.
}

==> sections/list_of_work_to_be_done.tex <==
\subsection{Things we have already done and data is available}
\begin{itemize}
    \item \textbf{Oversubscription}: We oversubscribed GPU while running multiple instances of ResNet-50. We started with ResNet-50 with 25\% instances and increased the number of instance from 1 to 8. Thus, oversubscribing GPU till 200\%. Similar experiment was done with instances of 50\% GPU. In both cases we saw latency growing rapidly after GPU was subscribed by more than 100\%. 
    
    \item \textbf{Division of GPU with multiple instance of} of ResNet-50 IF: For batch of 1,2,4,8 16, we have divided GPU with 1,2,3,...,N (N<=10) instance of ResNet-50 with 100/N\% GPU for each instance and measured throughput. In all batch size we see that throughput increases with increase in number of instances till N=5.i.e. when each instance is 20\%. 
    \item We followed up the over-subscription experiment with SLO of 50ms. And saw similar result.
    \item \textbf{Overprovisioning}: We over provisioned GPU till 500\% (By launching more instance of ResNet-50). We saw the throughput increases till 300\% (With increase in latency) but stops increasing after 300\%. (only latency keeps rising)-- this is also oversubscription... \textbf{I put the experiment description in oversubscription. }
    \item \textbf{Streams}: Right number of streams. Some models show benefit with 3 streams (Alexnet) while others do not show benefit with even 2 streams eg (VGG19). We could show MPS with spatial sharing is better alternative to stream.
    \item \textbf{Zero Copy GPU transfer (NetML)}: NetML shows both throughput improvement as well as CPU cycles reduction in transferring data to GPU.
    \item \textbf{Max-Min Allocation}: We have algorithm for Max-Min allocation. However, results are for only 2 IF coming up. We need to demonstrate with more than 2 IFs.
    \item \textbf{Notification from GPU}: comparison across  alternative methods of notification from the GPU to the CPU or to other GPU models (e.g., chaining) on the GPU of individual task completion  
\end{itemize}

\subsection{Things we have discussed that could go into next paper. Based on phone conversations}
\begin{itemize}
    \item \textbf{Limits on Parallelism of DNN:}  \textbf{Model wise limitation}: When a model is so small that increasing GPU\% do not reduce its latency anymore (eg. Alexnet) We could profile to see what causes the limits to parallelism in those cases. \textbf{Hardware wise:} We can check experimentally in NVPROF profile to see when a certain Kernel takes longer time to execute when we increase the batch size (as it has spawn more threads than GPU can run concurrently).
    \item\textbf{NetML in multiple GPUs}: If we are running multi GPU system but only 1 core of CPU is handling data transfer to all GPUs. We could potentially be doing a lot of work transferring data to GPU. NetML could help even more in these cases.
    \item Related to NetML. Most of our experiments were in images, thus, requiring around 500 packets for each image. A class of DNN such as translation can infer every packet. We can see impact of NetML in such case. 
    \item \textbf{Autoscaling}: Checking the oversubscription value of an IF, we can see when would be a good time to add or remove an IF instance. The goal is to have right amount of instances to fully utilize the GPU.
    \item \textbf{Using multiple GPUs}: Extending autoscaling to not only 1 GPU but making it able to run in multiple GPUs.
    \item \textbf{Model load time}: we have model load time (loading from disk or memory and getting ready to infer) in TensorRT, PyTorch and CNTK. We could extend our "Parameter sharing" to multi GPU scenario. GPU-to-GPU transfer of data can be done via PCIe-PCIe transfer. GPU runtime is still involved to facilitate the transfer of data but we can try NetML like approach to transfer models to another GPU as multiple GPU share same address space due to Unified Virtual Addressing. 
\end{itemize}
\subsection{Other things we discussed for either this paper or future long term work}
\begin{itemize}
    \item \textbf{Chain of ML functions}: Chaining ML functions across single or multiple GPU or multiple Compute Nodes.
    \item \textbf{Spatio Temporal Scheduling}: Spatio-temporal scheduling. We can then over-provision the GPU and still relay on temporal scheduling to concurrently execute two applications that can fit in GPU without interference.
    \item \textbf{Optimization Formulation for Batch Size:} Optimization formulation to show the batch size we produce with SLAB is close to optimal batch size.
    \item\textbf{Power consumption}: check if we are energy efficient using GSLICE or component of GSLICE rather than inferring without GSLICE. Power can be measured by GPU sensor itself. Energy spent per application unit. 
    \item \textbf{effective batch size for certain GPU\%}: we have a plot showing some batch size are more efficient at some GPU\%.
\end{itemize}

==> sections/rewrites.tex <==
\knote{should this part come before the "Measurement with ML models" part? Because that mainly uses CSS.}
\noindent\textbf{Selecting Spatial Sharing Method}: Alternative methods of spatial sharing of the GPU, namely, CUDA Streams and CUDA Multi-process Service (MPS) do not allow operator to specify the resources for each DNN model. Furthermore, we as well as other studies~\cite{other papers, GSLICE} have observed models interfering with each other's execution while multiplexing with CUDA streams and default CUDA MPS, leading to higher and unpredictable inference latency. Meanwhile, CSS provides resource isolation among the multiplexing DNNs, thus, avoids interference and provides predictable latency for each inference. Therefore, we chose to utilize CSS to provide spatial sharing for our ST-FD scheduler.



We evaluated different options: Streams; CUDA Multi-process Service (MPS) and Controlled Spatial Sharing (CSS)~\mbox{\cite{GSLICE}}, for spatial sharing of a NVIDIA Volta GPU. %for both  
%to understand one that would be suitable for high 
%throughput and latency of inference. We studied . 
%CUDA Streams has been available for NVIDIA GPUs for several generations, while CUDA MPS and CSS are more recent (NVIDIA Volta and newer). 
We spatially shared the GPU among 3 Alexnet instances to  concurrently infer requests, and show the models' mean and $99^{th}$ percentile (P-99) latency and average throughput in Table~\mbox{\ref{tab:streams_vs_css}}.
The models interfere with each other, inefficiently utilizing GPU with Streams and MPS resulting in higher latency (P-99 higher than mean, indicating unpredictability) even when spatially sharing GPU with the same DNN model. 
%The P-99 latency is higher than mean, indicating more unpredictable inference latency while inferring with Streams and MPS. 
On the other hand, CSS's GPU compute resource isolation and allocation of a Knee\% for Alexnet gives lower latency and 1.5$\times$ higher throughput than Streams and 1.1$\times$ higher than default MPS. CSS's mean and P-99 latency are close, indicating very predictable inference times. Thus, we choose CSS to provide spatial sharing for our ST-FD scheduler.\Scut{ spatially multiplex DNNs on GPUs.}\looseness-1


\noindent\textbf{Dynamic GPU Resource Reconfiguration without Downtime}:\label{sec:dynamic_gpu_recon1}
We observed that the GPU\% of a given model might need to be changed dynamically when working with different workloads of requests to models multiplexed on a GPU. However, due to the limitation of CUDA MPS~\mbox{\cite{nvidiamps2019}} to configure the GPU\% any GPU resource readjustment requires us to spin up a new CPU process with an updated GPU\%, which results in several seconds of downtime (depending on the ML framework initialization).
We utilize the overlapped execution approach of~\mbox{\cite{GSLICE}}, which maintains an \textit{active-standby} pair of process, where, an active process keeps processing incoming request while standby process loads DNN model into GPU with updated GPU\% and takes over inference when ready.
\Scut{
to mask the DNN loading and setup time while changing the GPU\%. We maintain a \textit{active-standby} pair of process, where the active process performs DNN inference in GPU. The standby process is a hot replica that loads all required software libraries for the DNN model but does not access the GPU (no need to set a GPU\%). When a GPU\% change is desired active process sends a message to standby to start loading the model, while, the active DNN instance continues processing requests until the standby process loads the DNN model on the GPU with a new GPU\% and is ready to infer.\looseness-1\Scut{ Once the standby is ready, it seamlessly takes over the inference and the original instance terminates.}
}
%\knote{up to here it is all GSLICE.}
%However, we should note that, 
But, while changing the GPU\%, two instances of the same model, the original and the new model,\Scut{loaded with a new GPU\% are running concurrently} 
occupy the GPU for a brief time during overlap. This increases the GPU memory demand. We overcome this drawback through  DNN parameter sharing.\Scut{by the model in the GPU  to run in the GPU as each instance of the model loads its own model parameters\Scut{ and creates its own buffers }in GPU. We explain }\Scut{ explained
%thus reducing memory required during resource reconfiguration \Scut{this effect of doubling of memory }
in \S~\ref{sec:dynamic_gpu_recon2}.To counter the increased GPU memory requirement while loading a new model with a different GPU\%
we share DNN parameters and other buffers between the original and new model.} As model parameters remain the same in both models, \revise{we separately load model parameters using an orchestrator process} and create cudaIPC handles for those parameter buffers.\Scut{create cudaIPC handles for all the parameter buffers of the original model and} When a new model instance is loaded with a new GPU\%, \revise{it forgoes copying the model parameters from CPU to GPU. The orchestrator process passes the cudaIPC handles to the new DNN instance, which then uses the handles to utilize the model parameters for inference. }
%similar to%~\cite{GSLICE}.
%\knote{so is this all GSLICE??}
Parameter sharing reduces the memory required by the newly loaded DNN model by up to 40\%, depending on size of the model's parameters. Thus, we not only avoid idling the GPU but also maintain a low GPU memory profile and thus run larger DNN models.\looseness-1





